Lazy Receding Horizon A* for Efficient Path Planning in Graphs with Expensive-to-Evaluate Edges

Motion-planning problems, such as manipulation in cluttered environments, often require a collision-free shortest path to be computed quickly given a roadmap graph. Typically, the computational cost of evaluating whether an edge of the roadmap graph is collision-free dominates the running time of search algorithms. Algorithms such as Lazy Weighted A* (LWA*) and LazySP have been proposed to reduce the number of edge evaluations by employing a lazy lookahead (one-step lookahead and infinite-step lookahead, respectively). However, this comes at the expense of additional graph operations: the larger the lookahead, the more the graph operations that are typically required. We propose Lazy Receding-Horizon A* (LRA*) to minimize the total planning time by balancing edge evaluations and graph operations. Endowed with a lazy lookahead, LRA* represents a family of lazy shortest-path graph-search algorithms that generalizes LWA* and LazySP. We analyze the theoretic properties of LRA* and demonstrate empirically that, in many cases, to minimize the total planning time, the algorithm requires an intermediate lazy lookahead. Namely, using an intermediate lazy lookahead, our algorithm outperforms both LWA* and LazySP. These experiments span simulated random worlds in $\mathbb{R}^2$ and $\mathbb{R}^4$, and manipulation problems using a 7-DOF manipulator.

==> lem1_proof_w_beta.tex <==
\begin{proof}
Since the algorithm has evaluated the edge~$(v_0,v)$ to be collision free, there exists a path $P = (v_{\rm{start}},\ldots,v_1,v_0,v)$ for which all edges were found to be collision free by  $\ab$. Assume there exists another collision-free path $P' = (v_{\rm{start}},\ldots,v_1',v_0',v)$ from $v_{\rm{start}}$ to $v$ such that $w(P') < w(P)$. 

Consider the iteration before $\ab$ evaluates $(v_0,v)$ 
and let 
$(v_{\beta - 1},v_{\beta - 2},\ldots,v_1,v_0,v)$ be the sequence of vertices along the $\beta$ edges leading to $v$ on $P$. 
Since the edge $(v_0,v)$ is evaluated,
there exists 
a border node~$\tau_i$ associated with $v_i$ where $0 \leq i \leq \beta-1$ and 
a frontier node $\tau$ that is $\alpha$ edges away from $\tau_i$ for which $\bar{w}(P[\tau])$ is minimal.

Let $\tau_j'$ be the last border node on $P'$ and 
let~$\tau'$ be the frontier node that is $\alpha$ edges away from $\tau_j'$ for which~$\bar{w}(P[\tau'])$ is minimal.
Note that since $(v_0,v)$ was evaluated, we have that $\bar{w}(P[\tau])$ is minimal which implies that $\bar{w}(P[\tau]) < \bar{w}(P[\tau'])$.
Finally, let $v_i$ and~$v_j'$ be the vertices associated with border nodes $\tau_i$ and $\tau_j'$, respectively.
% and
%let $u$ and $u'$ be the vertices associated with frontier nodes $\tau$ and $\tau'$, respectively.

Consider the following cases:
\begin{itemize}
	\item[C1] 	\textbf{We have that} $\bm{j > \alpha }$.
				Namely,  vertex $v_j'$ lies more than~$\alpha$ edges before~$v$. 
			Thus, the vertex $v'$ associated with frontier node $\tau'$ lies on $P'$ before $v$.
			By the assumption that $w(P')<w(P)$, we have that $\bar{w}(P[\tau']) < \bar{w}(P[\tau])$ which gives a contradiction to the fact that $\bar{w}(P[\tau]) < \bar{w}(P[\tau'])$.
				See Fig.~\ref{fig:C1}.
%
	\item[C2] 	\textbf{We have that} $\bm{\alpha \geq j}$.
				Namely,  vertex $v_j'$ lies at most~$\alpha$ edges before~$v$. 
			Thus, the vertex $u'$ associated with frontier node $\tau'$ is $v$ or a descendant of $v$.
			Consider the node~$\tau_v$ associated with vertex $v$.
			Clearly, $\tau_v$ is at most $\alpha$ edges from both border nodes $\tau_i$ and $\tau_j'$.
			By the assumption that $w(P')<w(P)$, we have that $\tau_v$ will have $\tau_i$ as it's ancestor in $\calT$ and \emph{not} $\tau_j'$ which contradicts the fact that $(v_0,v)$ is chosen for evaluation.
				See Fig.~\ref{fig:C2}.

\end{itemize}	
\end{proof}

\begin{figure*}	
	\centering
	\begin{subfigure}[t]{0.3\textwidth}
		\centering
		\includegraphics[height = 4.2cm]{correctness_C1.pdf}
		\caption{Case C1.}\label{fig:C1}		
	\end{subfigure}
	\quad
	\quad
	\begin{subfigure}[t]{0.3\textwidth}
		\centering
		\includegraphics[height = 4.2cm]{correctness_C2.pdf}
		\caption{Case C2.}\label{fig:C2}
	\end{subfigure}
%	\quad	
%	\begin{subfigure}[t]{0.3\textwidth}
%		\centering
%		\includegraphics[height = 4.2cm]{correctness_C3.pdf}
%		\caption{Case C3.}\label{fig:C3}
%	\end{subfigure}
%%
	\caption{Different cases considered in the proof of Lemma~\ref{lem:correctness}.}\label{fig:1}
\end{figure*}

